MixNN: A design for protecting deep learning models

In this paper, we propose a novel design, called MixNN, for protecting deep learning model structure and parameters. The layers in a deep learning model of MixNN are fully decentralized. It hides communication address, layer parameters and operations, and forward as well as backward message flows among non-adjacent layers using the ideas from mix networks. MixNN has following advantages: 1) an adversary cannot fully control all layers of a model including the structure and parameters, 2) even some layers may collude but they cannot tamper with other honest layers, 3) model privacy is preserved in the training phase. We provide detailed descriptions for deployment. In one classification experiment, we compared a neural network deployed in a virtual machine with the same one using the MixNN design on the AWS EC2. The result shows that our MixNN retains less than 0.001 difference in terms of classification accuracy, while the whole running time of MixNN is about 7.5 times slower than the one running on a single virtual machine.

==> tex/conclusion.tex <==
\section{Conclusion}
MixNN is a novel design for protecting model privacy. It divides a whole DL model to several parts, every part owns its private part of models and parameters. This part in MixNN is a layer in a DL model, and all layers are fully decentralized and constructed as a cascade. Besides the structure above, MixNN utilizes the method from mix network to hide the detailed communication address. Meanwhile, layer parameters and operations, and forward as well as backward message flow among non-adjacent layer are also hidden. In the experiment, we compare MixNN with MLP and show that MixNN retains the almost same performance in terms of classification accuracy. Because MixNN spends time on transferring message between servers (layers), encrypting and decrypting message with a large size, and packing the messages in one iteration with two times, the running time of MixNN becomes larger. 

==> tex/todo.tex <==
\section{Todo}
\chao{1. This model privacy is for training or prediction? Most papers are for the predictions.

2. The experiments. VGG -7

3. should we do the verification of the mix-learning?
}


